Quantifying Hypothesis Space Misspecification in Learning from Human-Robot Demonstrations and Physical Corrections

Human input has enabled autonomous systems to improve their capabilities and achieve complex behaviors that are otherwise challenging to generate automatically. Recent work focuses on how robots can use such input - like demonstrations or corrections - to learn intended objectives. These techniques assume that the human's desired objective already exists within the robot's hypothesis space. In reality, this assumption is often inaccurate: there will always be situations where the person might care about aspects of the task that the robot does not know about. Without this knowledge, the robot cannot infer the correct objective. Hence, when the robot's hypothesis space is misspecified, even methods that keep track of uncertainty over the objective fail because they reason about which hypothesis might be correct, and not whether any of the hypotheses are correct. In this paper, we posit that the robot should reason explicitly about how well it can explain human inputs given its hypothesis space and use that situational confidence to inform how it should incorporate human input. We demonstrate our method on a 7 degree-of-freedom robot manipulator in learning from two important types of human input: demonstrations of manipulation tasks, and physical corrections during the robot's task execution.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> algorithmic_approach.tex <==
\section{Algorithmic Approach}
\label{approach}

\begin{itemize}
    \item Although the proposed formalism enables us to capture if the robot's hypothesis space cannot well-explain the human's input, it is non-trivial to implement tractably for continuous $\beta, \weight$ and state and action spaces. Thus, we focus on two approximation schemes for two common forms of human input.
    \item Specifically, we discuss the algorithmic approach for two common domains for learning from human input: learning from demonstrations and from physical corrections.
    \item Before diving into the details of each domain, we note that for the rest of the paper we commit to reward functions that are linear, following the results in \cite{Ng2000inverse}:
    
    \begin{equation}
    \begin{aligned}
        \cost_{\weight}(\xtraj^{0:T}, \utraj_R^{0:T}, \utraj_H^{0:T}) =& ~\sum_{i=1}^d \weight^i \sum_{t=0}^T \statefeat_i(\state^t, \control_R^t, \control_H^t) \\ =& ~\weight^T\trajfeat(\xtraj^{0:T}, \utraj_R^{0:T}, \utraj_H^{0:T}),
    \label{eq:linear_cost}
    \end{aligned}
    \end{equation}
    
    where $\statefeat_i$ are fixed, known, bounded basis function mappings to $\mathbb{R}$, $\weight$ is the unknown parameter that the robot is trying to fit according to the human's preferences, and $d$ is the dimensionality of its domain, $\wspace$.
    \item In the presented domains, the functions $\statefeat_i: \mathbb{R}^n \times \uset \times \uset \rightarrow \mathbb{R}$ represent feature maps which encode \andreanote{write more here -- i stopped reading here.}
    \item It is important to stress that the model misspecification issue we are trying to mitigate is quite general and does not exclusively affect objectives based on hand-crafted features: any model, by definition, will ultimately fail to capture the underlying motivation of some human actions. 
    \item While it may certainly be possible, and desirable, to continually increase the complexity of the robot's model to capture a richer space of possible objectives, there will still be a need to account for the presence of yet-unlearned components of the true objective. In this sense, our work is complementary to open-world objective modeling efforts.
\end{itemize}

\subsection{Demonstrations}
\begin{itemize}
    \item Imagine a robot arm performing a household task, like moving a cup from the shelf onto your kitchen table. The robot wants to learn from a person's demonstrations how to best perform the task. For this purpose, the person gives one or a few demonstrations from which the robot infers the hidden reward function.
    \item Formally, in the case of learning from demonstrations, the human directly controls the robot's trajectory $\xtraj^{0:T}$ through her control input $\utraj_H^{0:T}$, which enables her to offer the robot a demonstration of how to perform the task at hand.
    \item During the demonstration, the robot is put in gravity compensation mode, to grant the person full control over her desired trajectory. As such, in this setting, the cost function $\cost_\weight$ does not depend on the robot controls $\utraj_R$.
    \item Additionally, since the person is primarily concerned with the quality of her demonstrated trajectory $\xtraj$ and not with the inputs required to achieve that demonstration, we make the assumption that the human's internal preferences are independent of her given control inputs $\utraj_H$. 
    \item Accordingly, the cost function in \eqref{eq:linear_cost} becomes:
    
    \begin{equation}
    \begin{aligned}
        \cost_{\weight}(\xtraj^{0:T}) = \weight^T\trajfeat(\xtraj^{0:T}).
    \label{eq:demo_cost}
    \end{aligned}
    \end{equation}

    \item We would like the robot to explicitly reason about the reliability of its human model given new inputs in the form of demonstrations. Given the above cost formulation, we can use the model in \eqref{eq:boltzmann}, which becomes:

    \begin{equation}
    \begin{aligned}
      P(\xtraj^{0:T} \mid \weight,\beta) =& \frac{e^{-\beta \weight^T \trajfeat(\xtraj^{0:T})}}{\int_{\bar{\xtraj}^{0:T}}e^{-\beta \weight^T \trajfeat(\bar{\xtraj}^{0:T})}d\bar{\xtraj}^{0:T}}.  
    \label{eq:demo_boltzmann}
    \end{aligned}
    \end{equation}

    \item Note that this equation is overparametrized, meaning that $\forall (\weight,\beta)$ pair with $\weight \in \wspace$ and $\beta \in [0,\infty)$ , one can always find a different $\weight' = c\weight$ with an associated $\beta' = \beta/c$.
    
    \item In order to be able to compare different $(\weight,\beta)$ pairs without confounding the overparametrization, we restrict our $\wspace$ to the set of vectors with norm 1. In this sense, we can think of $\weight$ as the direction of the human's intent and of $\beta$ as its magnitude.
    
    \begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/weight_sphere.jpg}
    \caption{\abnote{
    Draw a unit sphere representing the space of $\wspace$ to provide intuition for the interaction between $\weight$ and $\beta$:
    \begin{itemize}
        \item draw a vector larger than the sphere and show that the vector with norm 1 is $\weight$ and the magnitude of the large vector is $\beta$ - this is a demonstration with high situational confidence;
        \item draw another short vector and show that the vector with norm 1 is $\weight$ and the magnitude of the small vector is $\beta$ - this is a demonstration with low situational confidence.
    \end{itemize}}}
    \label{fig:weightsphere}
    \end{figure}
    
    \item Fig. \ref{fig:weightsphere} illustrates the intuition behind this modeling choice. When the robot is presented with a human demonstration, it can infer a $\weight$ vector on the unit sphere, signifying the person's preferences in her input. If the situational confidence in their demonstration is high, the robot infers a high magnitude vector of preferences. However, if the robot is not confident in the person's input, it will infer a low magnitude $\beta$. \abnote{this is not a great explanation; I need to write a better one that includes the intuition behind why low betas give uniform probability over all thetas in the hypothesis space}

    
    \item Given the model in \eqref{eq:demo_boltzmann}, we can easily obtain the joint posterior probability of the $(\weight, \beta)$ pair after observing a demonstrated trajectory:
    \begin{equation}
        P(\weight, \beta \mid \xtraj^{0:T}) = \frac{P(\xtraj^{0:T} \mid \weight,\beta)P(\weight,\beta)}{\int_{\bar{\weight},\bar{\beta}}P(\xtraj^{0:T} \mid \bar{\theta},\bar{\beta})P(\bar{\theta},\bar{\beta})d\bar{\theta}d\bar{\beta}}.
    \label{eq:posterior}
    \end{equation}
    
    \item Notice that equations \eqref{eq:demo_boltzmann} and \eqref{eq:posterior} constitute a doubly-intractable system with denominators that cannot be computed exactly. 
    
    \item Our solution to this problem consists in discretizing the space to integrate over.
    
    \item For the first intractability in \eqref{eq:demo_boltzmann}'s denominator, we chose to discretize the trajectory space to approximate the integral as a summation :
    $$\int_{\bar{\xtraj}^{0:T}}e^{-\beta \weight^T \trajfeat(\bar{\xtraj}^{0:T})}d\bar{\xtraj}^{0:T} \approx \sum_{\bar{\xtraj}^{0:T}\in \Xi_D}e^{-\beta \weight^T \trajfeat(\bar{\xtraj}^{0:T})}$$
    
    \item Here, $\Xi_D$ is a subset of the full trajectory space chosen to make the computation of the partition function tractable. We sampled 1500 trajectories to approximate this integral. We found that the most suitable way to sample trajectories was to sample, instead, $(\weight,\beta)$ pairs that the trajectory optimizer could use to compute optimal trajectories given those parameters. \abnote{should i say this in the case study section?}
    \item For the second intractability in equation \eqref{eq:posterior}, we also discretized the space of $\weight$ and $\beta$, which leaves us with a finite, easy to compute posterior.
    \item For the $\wspace$ discretization, we chose vectors in the positive quadrant of the unit sphere.
    \item In order to discretize situational confidence, we found that $\beta\in \{0.01,0.03,0.1,0.3,1.0, 3.0, 10.0, 30.0, 100.0\}$ was a suitable suitable range for our experimental purposes.
    
    \item Using the above discretization, we can now perform tractable inference to obtain a discrete posterior $b(\weight,\beta)$. Fig. \ref{fig:simulated_demo} exemplifies an intuitive explanation of the interaction between $\weight$ and $\beta$ given different human demonstrations. 
    
    \item In these examples, the robot's hypothesis space includes three features: efficiency in the form of sum of squared velocities over the trajectory, keeping the cup close to the table, and keeping the cup away from the laptop depicted in black. We illustrate the result of our inference algorithm for a correctly specified simulated demonstration, a noisy human demonstration, and a misspecified simulated demonstration. The posterior belief is shown for the combination of discrete parameters $\weight$ and $\beta$. Higher $\beta$ values indicate higher situational confidence. The three circles under each column represent the $\weight$ vector for that column, with the components being the efficiency, distance from the table, and distance from the human features. The proportion of each feature weight in the candidate $\weight$ vector is given by the opacity of the dark circle. 

    \item In \ref{spec}, the demonstration was an optimal trajectory produced with our out-of-the-box trajectory optimizer, in order to eliminate any noise that human demonstrations inevitable present. In this example, the objective was to carry the mug from the start configuration until the end, while keeping the mug close to the table. Notice that, with a perfect demonstration, the posterior distribution has no trouble finding the correct $\weight$ parameter, with the highest available confidence $\beta$.
    
    \item Next, we present a real noisy human demonstration to compare how the noise introduced affects the robot's inference. Notice that even with an imperfect demonstration, the robot is able to identify the correct $\weight$ parameter, but with a lower confidence $\beta$.
    
    \item Lastly, we present an optimal trajectory produced with out trajectory optimizer, but for an objective that is outside of the robot's hypothesis space: keeping the mug away from the human's body. Immediately we observe that the probability distribution is spread over all the $\weight$ values in the space, with the highest values on low $\beta$s. This example shows how, in the case of misspecified input, the robot's inference is unsure which objective the human had in mind, and assigns low situational confidence to the given input.
    
\begin{figure}
    \subfloat[(Left) Simulated perfect demonstration with the objective to keep the cup close to the table. (Right) Posterior belief resulted from this demonstration. Notice that a perfect demonstration leads to a high probability on the correct $\weight$ and high values for $\beta$.\abnote{change scale numbers to 0,0.15,.3}]{\label{spec}\includegraphics[width=\columnwidth]{figures/simulated_examples_1.png}} \\
    \subfloat[(Left) Noisy human demonstration with the objective to keep the cup close to the table. (Right) Posterior belief resulted from this demonstration. Notice that a noisy but correctly specified demonstration leads to a high probability on the correct $\weight$ and moderately high values for $\beta$. However, the noise in the demonstration significantly reduces the intensity of the probability at the distributional peak.]{\label{noisy}\includegraphics[width=\columnwidth]{figures/simulated_examples_2.png}}
    \\
    \subfloat[(Left) Simulated perfect demonstration with the objective to keep the cup away from the human’s body. (Right) Posterior belief resulted from this demonstration. Notice that, since this demonstration is misspecified (the robot is not reasoning about distance from the human), the posterior belief is spread out approximately uniformly over all $\weight$s and the lowest $\beta$ values. This indicates that the robot cannot tell what the demonstration was intended to teach it.]{\label{misspec}\includegraphics[width=\columnwidth]{figures/simulated_examples_3.png}}
    \caption{Three examples of demonstrations and the inferred posterior belief after each one of them. The robot infers the right $\weight=[0,1,0]$ from the two correctly specified demonstrations, but, unlike the perfect simulated demonstration in \ref{spec}, the noisy one in \ref{noisy} cannot reach the highest beta and has as overall more spread-out probability distribution with a lower peak value. Lastly, the perfect simulated demonstration that is misspecified in \ref{misspec} results in a posterior that is spread-out over all $\weight$s and the lowest $\beta$s , consistent with the robot not being able to tell what the human’s objective was.}
    \label{fig:simulated_demo}
\end{figure}
    
    \item Section \ref{case_study} expands the above example to a larger-scale offline experiment with real human demonstrations. We will show that our method reliably identifies the correct objective when the input is correctly specified, and consistently infers low situational confidence for misspecified inputs. 
    \item Note that in situations where the designer might want high fidelity inference over a large space of $\weight$ vectors, reasoning over a heavily discretized space would be more computationally expensive. Since in our learning-from-demonstrations scenario the inference happens offline, after providing the robot with human demonstrations, we are not concerned with having a real-time inference algorithm.
    \item However, in the next section which focuses on human input provided in the form of physical corrections during the robot's task execution, having an inference algorithm that can run in real-time is critical. We will present an online version of our situational confidence framework.

\end{itemize}

\subsection{Corrections}

\begin{itemize}
    \item We now consider settings where a robot is collaborating with a person to perform everyday tasks by learning from pHRI, but their feature spaces might not be shared. When the robot receives human input, it should be able to reason about the situational confidence given by their action and replan its trajectory accordingly. \abnote{I replaced relevance with situational confidence, although we do define relevance in the paper later as part of the approximation.}
\end{itemize}

\subsubsection{A Graphical Model for Correction Relevance}

\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\textwidth]{figures/graphical_model.pdf}
\caption{(a) \abnote{WE NEED TO CHANGE THIS.} In the complete graphical model, $u_H$ is an observation of the true objective ($\theta$) and rationality coefficient ($\beta$);
inference over $\theta$ is intractable.(b) We use the proxy variable $\Phi(\xi_H)$ to first estimate $\beta$. (c) We interpret the estimate $\hat{\beta}$ as an indirect observation of the unobserved $r$, which we then use for the $\theta$ estimate.}
\label{fig:graphical_models}
\end{figure*}

\begin{itemize}
    \item In the physical corrections setting, the robot starts with an initial guess of the parameter $\weight$ and computes the optimal trajectory with respect to the current objective $\cost_\weight$. 
    \item The robot performs the task at hand by applying controls $\utraj_R^{0:T}$ via an impedance controller in order to track the found trajectory $\xtraj^{0:T}$. 
    \item At any timestep $t$ during the trajectory execution, the human may physically interact with the robot, inducing a joint torque, $\control_H^t$.
    \item When this happens, the robot can use the human input to update its $\weight$ parameter, which in turn updates the objective for the rest of the task.
    \item Given the new adapted objective, the robot replans an optimal trajectory $\xtraj^{0:T}$ and tracks it until the next input is sensed or until the task is completed.
    \item Notice that, since the trajectory optimizer we use intrinsically finds the optimal robot controls $\utraj_R^{0:T}$ to produce $\xtraj^{0:T}$, the cost function in \eqref{eq:linear_cost} does not explicitly depend on $\utraj_R^{0:T}$.
    \item Since the person sporadically gives a correction $\control_H$ whenever necessary, we assume that the cost function the robot considers at a particular timestep relies on the specific human control applied at that timestep. \abnote{rewrite these past two points because they're not great}
    \item Additionally, we follow \cite{bajcsy2017phri} in formulating the crucial assumption that, when giving physical corrections, the person is trying to be informative while minimizing effort. This results in an additional regularization term that penalizes the magnitude of the human control $\control_H^t$.
    \item Encompassing these assumptions, the cost function in \eqref{eq:linear_cost} becomes:
    
    \begin{equation}
    \begin{aligned}
        \cost_{\weight}(\xtraj^{0:T}, \control_H^t) = ~\weight^T\trajfeat(\xtraj^{0:T}, \control_H^t) + \lambda\|\control_H^t\|^2.
    \label{eq:phri_cost}
    \end{aligned}
    \end{equation}
    
    \item  To compute the feature vector $\trajfeat(\xtraj^{0:T}, \control_H^t)$, we follow the approach in \cite{bajcsy2017phri} and introduce the notion of a \textit{deformed trajectory} $\xtraj_D^{0:T}$. This trajectory represents the human's desired trajectory that results from applying torque $\control_H$ onto the robot's current trajectory $\xtraj^{0:T}$.
    
    \item Given $\xtraj^{0:T}$ and $\control_H^t$, we compute $\xtraj_D^{0:T}$ by deforming the robot's current trajectory $\xtraj^{0:T}$ in the direction of $\control_H$:
    
    \begin{equation}
    \begin{aligned}
        \xtraj_D^{0:T} = \xtraj^{0:T} + \mu A^{-1}U_H,
    \label{eq:deformation}
    \end{aligned}
    \end{equation}
    
    where, $\mu>0$ scales the magnitude of the deformation, $A$ defines a norm on the Hilbert space of trajectories and dictates the deformation shape \cite{deformation}, and $U_H=\control_H$ at the current time and $U_H=0$ otherwise\footnote{We used a norm $A$ based on acceleration, consistent with \cite{bajcsy2017phri}, but other norm choices are possible as well.}. 
    
    \item We can rewrite \eqref{eq:phri_cost} in terms of the deformed trajectory:
    
    \begin{equation}
    \begin{aligned}
        \cost_{\weight}(\xtraj^{0:T}, \control_H^t) = ~\weight^T\trajfeat(\xtraj_D^{0:T}) + \lambda\|\control_H^t\|^2.
    \label{eq:phri_cost_deformed}
    \end{aligned}
    \end{equation}
    
    \item Overall, the intuition behind \eqref{eq:phri_cost_deformed} is that, when choosing actions, the human is modeled as trading off between inducing a good trajectory $\xtraj_D^{0:T}$ with respect to~$\weight$, and minimizing her effort. 
    
    \item  Equipped with this cost function, we would also like the robot to explicitly reason about the reliability of its human model given new inputs in the form of corrections. Remark that the person cannot give full demonstrations $\xtraj^{0:T}$, and, instead, can only offer corrections $\control_H^t$ after observing the robot's current trajectory $\xtraj^{0:T}$. As such, we modify the model in \eqref{eq:boltzmann} into a conditional form:

    \begin{equation}
        P(\control_H^t \mid \xtraj^{0:T} ; \weight, \beta) = \frac{e^{-\beta ({\weight}^\top\Phi(\xtraj_D^{0:T}) + \lambda\|\control_H^t\|^2)}}{\int e^{-\beta ({\weight}^\top\Phi(\bar{\xtraj}_D^{0:T}) + \lambda\|\bar{\control}\|^2)}d\bar{\control}}\enspace.
    \label{eq:boltzmann_phri}
    \end{equation}

    where $\xtraj_D^{0:T}$ and $\bar{\xtraj}_D^{0:T}$ are given by \eqref{eq:deformation} applied to their respective controls $\control_H^t$ and $\bar{\control}$.

\item Ideally, with this model of human actions we would perform inference over both the situational confidence $\beta$ and the parameters $\weight$ by maintaining a joint Bayesian belief $b(\weight, \beta)$. Similarly to the demonstrations case, our probability distribution over $\weight$ would automatically adjust for correctly specified corrections, whereas for misspecified ones the robot would stay closer to its prior on $\weight$: the robot would implicitly realize that there is a better $u_H$ for each possible $\weight$, and therefore no $\weight$ explains the correction. 

\item Unfortunately, this is not possible in real time given the continuous and possibly high-dimensional nature of the weight-space, $\wspace$. Even if we discretize the space $\wspace$ to make it tractable like we did in the demonstrations case, the inference procedure would still be too slow, making the method infeasible for use in the real-time collaborative scenarios that we are aiming for.

\item To alleviate the computational challenge of performing joint inference over $\beta$ and $\weight$, we introduce a binary variable $r \in \{0,1\}$ which (a) indicates interaction \textit{relevance}, and (b) allows us to split inference over $\beta$ and $\theta$ into two separate computations. When $r=1$, the interaction appears less noisy (i.e. $\beta$ is large) and the human's desired modification of the robot's behavior can be well explained by \emph{some} feature weight vector $\theta \in \Theta$. As a result, the interaction $\control_H^t$ is likely to be efficient for the cost encoded by this $\theta$. Conversely, when $r=0$, the interaction appears noisy (i.e. $\beta$ is small) and the person is correcting some feature(s) that the robot does not have access to. Thus, the interaction $\control_H^t$ is substantially less likely to be efficient for any cost expressible within the space $\Theta$.

\item Overall, this forms the graphical model in \ref{fig:graphical_models}a, with $P(\control_H^t \mid \xtraj^{0:T} ; \weight, \beta)$ defined above, and the distribution $P(\beta \mid r)$ (describing what $\beta$ we expect under relevant or irrelevant corrections) to be learned empirically. Next, we simplify the problem to enable real time computation while preserving the benefit of automatically adjusting the learning depending on relevance. 

\end{itemize}

\subsubsection{Approximate Inference} 

\begin{figure*}
\centering
  \centering
  \includegraphics[scale=.47]{figures/histograms_all.pdf}
  \caption{Empirical estimates for $P(\hat{\beta} \mid r)$ and their corresponding chi-squared ($\chi^2$) fits.}
  \label{fig:histograms}
\end{figure*}

\begin{itemize}
    \item We simplify inference by leveraging a proxy variable $\trajfeat(\xtraj_D^{0:T})$---the feature values of the corrected trajectory $\xtraj_D^{0:T}$---to split the problem into two stages. Rather than looking at how relevant $\control_H^t$ is overall, we first estimate the situational confidence $\beta$ (and therefore relevance $r$) based on how efficiently $\control_H^t$ produced the feature values of $\trajfeat(\xtraj_D^{0:T})$. If there is a more efficient correction that would induce $\trajfeat(\xtraj_D^{0:T})$, this suggests that the correction was not relevant to the robot's hypothesis space. Next, armed with an estimate of relevance, we infer $\weight$ from $\trajfeat(\xtraj_D^{0:T})$. 
    
\item These two steps are captured by the two simplified graphical models in Figure \ref{fig:graphical_models}b and Figure \ref{fig:graphical_models}c. 

\item The first relates $\control_H^t$ to $\beta$, $\xtraj^{0:T}$, and the induced feature values $\trajfeat(\xtraj_D^{0:T})$ by modeling that $\control_H^t$ should achieve the $\trajfeat(\xtraj_D^{0:T})$ feature values with minimal effort. This objective can be captured by the following cost function:

\begin{equation}
    \cost_{\trajfeat(\xtraj_D^{0:T})} (\bar\control) = \|\bar\control\|^2 + \lambda \|\trajfeat(\xtraj_D^{0:T}) - \trajfeat(\bar\xtraj_D^{0:T})\|^2,
\end{equation}

where $\lambda\|\trajfeat(\bar{\xtraj}_D^{0:T}) - \trajfeat(\bar\xtraj_D^{0:T})\|^2 $ is a strong penalty on deviating from the induced features.

\item Using a Boltzmann-like distribution for the human action, we obtain the following model:

\begin{equation}
%\resizebox{.5 \textwidth}{!} 
%{
	P(\control_H^t \mid \beta, \trajfeat(\xtraj_D^{0:T}), \xtraj^{0:T}) = \frac{e^{-\beta \|\control_H^t\|^2}}{\int e^{-\beta( \|\bar{\control}_H^t\|^2+ \lambda\|\trajfeat(\bar{\xtraj}_D^{0:T}) - \trajfeat(\xtraj_D^{0:T})\|^2 )}d\bar{\control}_H^t}
%}
	\label{eq:bayesnetb_model}
\end{equation}

where the numerator's penalty is 0 since the observed $\trajfeat(\xtraj_D^{0:T})$ is exactly the one induced by the given $\control_H^t$). Equation \eqref{eq:bayesnetb_model} will enable us to estimate a $\hat{\beta}$ from the observed $\control_H^t$.

\item The second simplified graphical model (Figure \ref{fig:graphical_models}c) relates the induced feature values $\trajfeat(\xtraj_D^{0:T})$ to $\weight$ as a function of the relevance. When $r=1$, the induced features should have low cost with respect to $\weight$; when $r=0$, the induced features \emph{do not depend on $\weight$}, and we model them as Gaussian noise centered at the current robot trajectory feature values:
\begin{equation}
P(\trajfeat(\xtraj_D^{0:T}) \mid \weight, r) = \begin{cases} \frac{e^{-\weight^\top\trajfeat(\xtraj_D^{0:T})}}{\int e^{-\weight^{\top}\trajfeat(\tilde{\xtraj}_D^{0:T})} d\tilde{\xtraj}_D^{0:T}} ,& r=1 \\ \left(\frac{\lambda}{\pi}\right)^\frac{k}{2} e^{-\lambda ||\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})||^2} ,& r=0 \end{cases}
\label{eq:bayesnetc_model}
\end{equation}
with the constant in the $r=0$ case corresponding to the normalization term of the normal distribution.

\item Finally, this graphical model also relates the estimated $\hat{\beta}$ from the first simplified model to $r$ by a $P(\hat{\beta} \mid r)$. We fit this distribution from controlled user interaction samples where we know $r$. For each sample interaction, we compute a $\hat{\beta}$ (using Equation \ref{eq:beta_map} below) and label it with the corresponding binary $r$ value. 

\item We fit a chi-squared distribution to these samples to obtain the probability distributions for $P(\hat{\beta} \mid r=0)$ and $P(\hat{\beta} \mid r=1)$. The resulting distribution fits are shown in Figure \ref{fig:histograms}.

\end{itemize}

\subsubsection{Estimating $\beta$} 

\begin{itemize}

\item The integral in Equation \ref{eq:bayesnetb_model} is computationally prohibitive, but we can approximate it via a Laplace approximation (detailed in Appendix \ref{app:laplace}): 

\begin{equation}
\begin{aligned}
	P(\control_H^t \mid \beta, \trajfeat(\xtraj_D^{0:T}), \xtraj^{0:T}) \approx \\  \frac{e^{-\beta(  \|u_H\|^2)}}{ e^{-\beta( \|{\control_H^*}\|^2 + \lambda\|\trajfeat(\xtraj_D^*) - \trajfeat(\xtraj_D^{0:T})\|^2)}}\sqrt{\frac{\beta^k|H_{\control^*_H}|}{2\pi^k}}
\end{aligned}
\enspace,
\label{eq:laplace}
\end{equation}
where $k$ is the action space dimensionality and $H_{\control_H^*}$ is the Hessian of the cost function around $\control_H^*$. We obtain the optimal action $\control_H^*$ by solving the constrained optimization problem: 

\begin{equation}
\begin{aligned}
& \underset{\control}{\text{minimize}}
& & \|\control\|^2 \\
& \text{subject to}
& & \trajfeat(\xtraj^{0:T}+\mu A^{-1}U) - \trajfeat(\xtraj_D^{0:T}) = 0.
\end{aligned}
\label{opt:optimal_uH}
\end{equation}

\item Notice that by formulating the problem as a constrained optimization, the $\lambda$-term in Equation \ref{eq:laplace} is close to 0 and vanishes, so the final conditional probability becomes:

\begin{equation}
	P(\control_H^t \mid \beta, \trajfeat(\xtraj_D^{0:T}), \xtraj^{0:T}) = e^{-\beta(\|\control_H^t\|^2-\|\control_H^*\|^2 )}\sqrt{\frac{\beta^k|H_{u^*_H}|}{2\pi^k}}\enspace.
\label{eq:laplace2}
\end{equation}

\item We can obtain an estimate of the rationality coefficient via a maximum likelihood estimate:

\begin{equation}
\begin{aligned}
	\hat{\beta} =& \arg\max_{\beta} \{\log(P(\control_H^t \mid \beta, \trajfeat(\xtraj_D^{0:T}))\} \\
	=& \arg\max_{\beta} \{-\beta(\|\control_H\|^2-\|\control_H^*\|^2 ) + \log(\sqrt{\frac{\beta^k|H_{\control^*_H}|}{2\pi^k}})\}
\end{aligned}
\end{equation}

and setting the gradient to zero:

\begin{equation}
	\hat{\beta} = \frac{k}{2(\|\control_H\|^2-\|\control_H^*\|^2)}\enspace.
\label{eq:beta_map}
\end{equation}

\item \noindent\textbf{Intuitive Interpretation of $\hat{\beta}$.} The estimator above yields a high value when the difference between $\control_H$ and $\control_H^*$ is small, i.e. the person's correction achieves the induced features $\trajfeat(\xtraj_D^{0:T})$ efficiently. For instance, if $\xtraj_D^{0:T}$ brings the robot closer to the table, and $\control_H$ pushes the robot straight towards the table, $\control_H$ is an efficient way to induce those new feature values. However, when there is a much more efficient alternative (e.g. when the person pushes mostly sideways rather than straight towards the table), $\hat{\beta}$ will be small. Efficient ways to induce the feature values will suggest relevance, inefficient ones will suggest irrelevance (i.e. there is something else that explains the correction).

\subsubsection{Estimating ${\weight}$}
Lastly, we can infer a new $\weight$ estimate based on the model from Figure  \ref{fig:graphical_models}c.
We do this tractably by interpreting the estimate $\hat\beta$ obtained from \eqref{eq:beta_map} as an indirect observation of the unknown variable $r$.
We empirically characterize the conditional distribution $P(\hat\beta\mid r)$, and then combine the learned likelihood model with an initial uniform prior $P(r)$ to maintain a Bayesian posterior on $r$ based on the evidence $\hat\beta$ constructed from human observations at deployment time, $P(r \mid \hat\beta) \propto P(\hat\beta \mid r) P(r)$.

\item Further, since we wish to obtain a posterior estimate of the human's objective $\weight$, we use the model from Figure  \ref{fig:graphical_models}c to obtain the posterior probability measure
\begin{equation}\label{eq:theta_from_beta_hat}
P(\weight \mid \trajfeat(\xtraj_D^{0:T}),\hat\beta) \propto \sum_{r \in \{0,1\} } P\big(\trajfeat(\xtraj_D^{0:T}) \mid \weight, r\big) P(r \mid \hat\beta) P(\weight)
\enspace.
\end{equation}

\item Following \cite{bajcsy2017phri}, we approximate the partition function in the human's policy  \eqref{eq:bayesnetc_model} by the exponentiated cost of the robot's original trajectory, thereby obtaining
\begin{equation}
P(\trajfeat(\xtraj_D^{0:T}) \mid \weight, r=1) = 
	e^{-\weight^\top\big(\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})\big)}\enspace. 
\label{eq:bayesnetc_with_constants}
\end{equation}

\item We also consider a Gaussian prior distribution of $\weight$ around the robot's current estimate $\hat\weight$:
\begin{equation}
P(\weight) = \frac{1}{(2\pi\alpha)^\frac{k}{2}} e^{-\frac{1}{2\alpha} ||\weight-\hat{\weight}||^2}
\enspace.
\end{equation}

\item The maximum-a-posteriori estimate of the human's objective $\weight$ is therefore the solution maximizer of

\begin{gather}\begin{aligned}\label{eq:posterior_theta}
P(\weight) \Big[ P(r=1 \mid \hat\beta)P\big(\trajfeat(\xtraj_D^{0:T})\mid\weight,r=1\big) + \\ + P(r=0 \mid \hat\beta)P\big(\trajfeat(\xtraj_D^{0:T})\mid \weight,r=0\big) \Big] \\
     = \frac{1}{(2\pi\alpha)^\frac{k}{2}}
e^{-\frac{1}{2\alpha}||\weight-\hat{\weight}||^2}
   \Big[ P(r=1 \mid \hat\beta) e^{-\weight^\top\big(\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})\big)}\\ + P(r=0 \mid \hat\beta) \left(\frac{\lambda}{\pi}\right)^\frac{k}{2} e^{-\lambda||\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})||^2}\Big]
\enspace.
\end{aligned}\end{gather}

\item Differentiating \eqref{eq:posterior_theta} with respect to $\weight$ and equating to 0 gives the maximum-a-posteriori update rule:
\begin{gather}\label{eq:theta_update}
\hat\weight' = \hat\weight - \alpha \frac{P(r=1 \mid \hat\beta) e^{-\hat\weight'^\top\big(\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})\big)}}
{P(r=1 \mid \hat\beta) e^{-\hat\weight'^\top\big(\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})\big)} +
P(r=0 \mid \hat\beta) \left(\frac{\lambda}{\pi}\right)^\frac{k}{2} e^{-\lambda||\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})||^2}}
\big(\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})\big)
\enspace.
\end{gather}

\item We note that due to the coupling in $\hat\weight'$, the solution to \eqref{eq:theta_update} is non-analytic and can instead be obtained via classical numerical approaches like Newton-Raphson or quasi-Newton methods.

\item In previous objective-learning approaches including \cite{bajcsy2017phri} and \cite{maxent}, it is implicitly assumed that all human actions are fully explainable by the robot's representation of the objective function space ($r=1$), leading to the simplified update
\begin{equation}\label{eq:corl_update}
\hat\weight' = \hat\weight - \alpha
\big(\trajfeat(\xtraj_D^{0:T})-\trajfeat(\xtraj^{0:T})\big)
\enspace,
\end{equation}
which can be easily seen to be a special case of \eqref{eq:theta_update} when $P(r=0 \mid \hat\beta)\equiv 0$.
Our proposed update rule therefore \emph{generalizes} commonly-used objective-learning formulations to cases where the human's underlying objective function is not fully captured by the robot's model.
We expect that this extended formulation will enable learning that is more robust to misspecified or incomplete human objective parameterizations. Once we obtain the $\hat{\weight}'$ update, we replan the robot trajectory in its 7-DOF configuration space with an off-the-shelf trajectory optimizer. We used TrajOpt \cite{trajopt}, which is based on sequential quadratic programming and uses convex-convex collision checking. 
\item \noindent\textbf{Intuitive Interpretation of $\hat{\weight}$.} The update rule changes the weights in the objective in the direction of the feature difference as well, but how much it does so depends on the probability assigned to the correction being relevant. At one extreme, if we know with full certainty that the correction is relevant, then we do the full update as in traditional objective learning. But crucially, at the other extreme, if we know that the correction is irrelevant, we do not update at all and keep our prior belief.

\end{itemize}

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Demonstrations}

\begin{itemize}
    \item We evaluated our method with human data collected offline.
    \item Independed and Dependent Variables.
    \item Hypotheses: 1) correctly specified interactions result in high $\beta$, misspecified interactions result in low $\beta$; 2) Not reasoning about how rational interactions and, instead, indiscriminately learning from every demonstration leads to significant unintended learning.
    \item explain the tasks; perhaps show a figure with what the tasks are?
    \item ANOVA Analysis
    \item Figure 8: Average $\beta$ for relevant and irrelevant interactions to demonstrate hypothesis 1. 
    \item Figure 9: Plot that demonstrated hypothesis 2. I'm not certain what that should be yet.
\end{itemize}

\subsection{Physical Corrections}

\abnote{Again, experiments pasted from the CoRL paper.}

\subsubsection{Offline $\beta$-estimation Experiments}
    
\begin{figure*}
\centering
  \centering
  \includegraphics[scale=.38]{figures/histograms_all.pdf}
  \caption{Empirical estimates for $P(\hat{\beta} \mid r)$ and their corresponding chi-squared ($\chi^2$) fits.}
  \label{fig:histograms}
\end{figure*}

We evaluate our rationality estimates with \emph{human data} collected offline.

\noindent\textbf{Independent and Dependent Variables.} We recruited 12 people to physically interact with a JACO 7DOF robotic arm as it moves from a start to a goal pose while holding a cup. We asked the participants to intentionally correct a feature (that the robot may or may not know about): adjusting the distance of the end effector from the table, adjusting the distance from the person, or adjusting the cup's orientation\footnote{Because users tend to accidentally correct more than one feature, we perform $\beta$-inference separately for each feature. This requires more overall computation (although still linear in the number of features and can be parallelized) and a separate $P(\hat{\beta} \mid r)$ estimate for each feature.
%In the future, we could resolve this problem by normalizing every feature.
}. 
In this data collection stage, the robot did not perform learning and simply tracked a predefined trajectory with impedance control \citep{impedance}. The participants were instructed to intervene only once during the robot's task execution, in order to record a single physical correction. 

Next, we ran our inference algorithm using the recorded human interaction torques and robot joint angle information. We measured what $\hat{\beta}$ would have been for each interaction if the robot knew about a given subset of the features. By changing the subset of features for the robot, we changed whether any given human interaction was \emph{relevant} to the robot's hypothesis space.

\noindent\textbf{Hypotheses:}

\noindent\textbf{H1.} \textit{Relevant interactions result in high $\hat{\beta}$, whereas interactions that change a feature the robot \textbf{does not} know about result in low $\hat{\beta}$ for all features the robot \textbf{does} know about.}
\vspace{-1mm}

\noindent\textbf{H2.} \textit{Not reasoning about relevant interactions and, instead, indiscriminately learning from every update leads to significant unintended learning.}

\noindent\textbf{Analysis.} 
We ran a repeated-measures ANOVA to test the effect of relevance on our $\hat{\beta}$. We found a significant effect ($F(1,521)=9.9093$, $p=0.0017$): when the person was providing a relevant correction, $\hat{\beta}$ was significantly higher. This supports our hypothesis H1.

FIGURE 10: Figure \ref{fig:beta_relevance} plots $\hat{\beta}$ under the relevant (orange) and irrelevant (blue) conditions. Whereas the irrelevant interactions end up with $\hat{\beta}$s close to 0, relevant corrections have higher mean and take on a wider range of values, reflecting varying degrees of human performance in correcting something the robot knows about. We fit per-feature chi-squared distributions for $P(\hat{\beta} \mid r)$ for each value of $r$ which we will use to infer $r$ and, thus, $\theta$ online. In addition, Figure \ref{fig:update_relevance} illustrates that even for irrelevant human actions $u_H$, the resulting feature difference $\Delta\Phi = \Phi(\xi_H)-\Phi(\xi_R)$ is non-negligible. This supports our second hypothesis, H2, that not reasoning about action relevance is detrimental to learning performance when the robot receives misspecified updates.

%\noindent\textbf{Fitting $P(\beta|r)$.}
%The significant distinction between $\beta$ values for relevant versus irrelevant actions allows us to fit distinct probability distributions to the samples we collected. In Figure \ref{fig:histograms} we fit $chi-$squared distributions for $P(\beta|r)$ for each feature, for both relevant and irrelevant actions, and we do, indeed, see discerning shapes within relevance pairs. We utilize these empirical estimates to obtain $P(r|\beta)$ via Bayes rule, which we can make use of for the gradient update procedure described in Equation \eqref{eq:gradient_adaptive}.

%\adnote{I think we should fit P(beta|r) on some subset of the samples; and then test how well we could classify r on a test set?}

%\vspace{-2mm}
\subsubsection{Online Learning User Study}

Our offline experiments suggested that $\hat{\beta}$ can be used as a measure  of whether physical interactions are relevant and should be learned from. Next, we conducted an IRB-approved user study to investigate the implications of using these estimates during learning. During each experimental task, the robot began with a number of incorrect weights and participants were asked to physically correct the robot. Locations of the objects and human were kept consistent in our experiments across tasks and users to control for confounds\footnote{We assume full observability of where the objects and the human are, as the focus of this paper is not sensing.}. The planning and inference were done for robot trajectories in 7-dimensional configuration space, accounting for all relevant constraints including joint limits and self-collisions, as well as collisions between obstacles in the workspace and any part of the robot’s body.\footnote{For video footage of the experiment, see: \href{https://youtu.be/stnFye8HdcU}{https://youtu.be/stnFye8HdcU}} 

\subsection{Experiment Design}

\noindent\textbf{Independent Variables.}
We used a 2 by 2 factoral design. We manipulated the pHRI learning strategy with two levels (fixed and adaptive learning), and also relevance (human corrected for features inside or outside the robot's hypothesis space). In the fixed learning strategy, the robot updated its feature weights from a given interaction via \eqref{eq:corl_update}. In the adaptive learning strategy, the robot updates its feature weights via \eqref{eq:theta_update}. The offline experiments above provided us an estimate for $P(r\mid \hat{\beta})$ that we used in the gradient update. 

\noindent\textbf{Dependent Measures.}

\textbf{\emph{Objective.}} To analyze the objective performance of the two learning strategies, we focused on comparing two main measurements: the length of the $\hat{\theta}$ path through weight space as a measurement of the learning process, and the regret in feature space measured by
$|\Phi(\xi_{\theta^*}) - \Phi(\xi_{actual})|$.

\textbf{\emph{Subjective.}} For each condition, we administered a 7-point Likert scale survey about the participant's interaction experience (Table \ref{tab:likert}). We separate the survey into 3 scales: task completion, task understanding, and unintended learning.

\begin{figure}[t!]%[!htbp]
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[height=.5\textwidth]	{figures/features_relevant_barplots.pdf}\\
\caption{Average $\beta$ for relevant and irrelevant interactions.}
 \label{fig:beta_relevance}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[height=.5\textwidth]{figures/update_relevant_barplots.pdf}\\
\caption{Average $\Delta\Phi$ for relevant and irrelevant interactions.}
 \label{fig:update_relevance}
\end{subfigure}
\vspace{1mm}
\caption{$\beta$ values are significantly larger for relevant actions than for irrelevant ones. Feature updates are non-negligible even during irrelevant actions, which leads to significant unintended learning for fixed-$\beta$ methods.}
\label{fig:offline_relevant}
\end{figure}

\noindent\textbf{Hypotheses:}

\textbf{H1.} \textit{On tasks where humans try to correct \textbf{inside} the robot's hypothesis space (relevant corrections), detecting irrationality is not inferior to assuming rational human behavior.}
\vspace{-1mm}

\textbf{H2.} \textit{On tasks where humans try to correct \textbf{outside} the robot's hypothesis space (irrelevant corrections), detecting irrationality reduces unintended learning.}
\vspace{-1mm}

\textbf{H3.} \textit{On tasks where they tried to correct \textbf{inside} the robot's hypothesis space, participants felt like the two methods performed the same.}
\vspace{-1mm}

\textbf{H4.} \textit{On tasks where they tried to correct \textbf{outside} the robot's hypothesis space, participants felt like our method reduced unintended learning.}


\noindent\textbf{Tasks.}
We designed four experimental household manipulation tasks for the robot to perform in a shared workspace. For each experimental task, the robot carried a cup from a start to end pose with an initially incorrect objective. Participants were instructed to physically intervene to correct the robot's behavior during the task. Similar to state-of-the-art methods, all the features were chosen to be intuitive to a human to ensure that participants could understand how to correct the robot.

In Tasks 1 and 2, the robot's default trajectory took a cup from the participant and put it down on the table, but carried the cup too high above the table. In Tasks 3 and 4, the robot also took a cup from the human and placed it on the table, but this time it initially grasped the cup at the wrong angle, requiring human assistance to correct end-effector orientation to an upright position. For Tasks 1 and 3, the robot knew about the feature the human was asked to correct for ($r=1$) and participants were told that the robot should be compliant. For Tasks 2 and 4, the correction was irrelevant ($r=0$) and participants were instructed to correct any additional unwanted changes in the trajectory.

\noindent\textbf{Participants.}
We used a within-subjects design and randomized the order of the learning methods during experiments. In total, we recruited 12 participants (6 females, 6 males, aged 18-30) from the campus community, 10 of which had technical backgrounds and 2 of which did not. None of the participants had experience interacting with the robot used in our experiments.

\noindent\textbf{Procedure.}
Every participant was assigned a random ordering of the two methods, and performed each task without knowing how the methods work. At the beginning of each task, the participant was shown the incorrect default trajectory, followed by the desired trajectory. Then the participant performed a familiarization round, followed by two recorded experimental rounds. After answering the survey, the participant repeated the procedure for the other method. %This process was repeated for every task. 

\vspace{-0.3cm}

\begin{figure}[t!]%[!htbp]
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[height=.5\textwidth]	{figures/average_delta_cost_barplots.pdf}\\
\caption{Regret averaged across subjects.}
 \label{fig:regret}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[height=.5\textwidth]{figures/average_weight_path_barplots.pdf}\\
\caption{$\hat{\theta}$ learning path length averaged across subjects.}
 \label{fig:weight_path}
\end{subfigure}
\vspace{0.5mm}
\caption{Comparison of regret and length of $\hat{\theta}$ learning path through weight space over time (lower is better).
}
\label{fig:delta_cost}
\end{figure}

\subsection{Analysis}

\noindent\textbf{Objective.}
We ran a repeated-measures factorial ANOVA with learning strategy and relevance as factors for the regret. We found a significant main effect for the method ($F(1,187)=7.8, p=0.0058$), and a significant interaction effect ($F(1,187)=6.77, p=0.0101$). We ran a post-hoc analysis with Tukey HSD corrections for multiple comparisons to analyze this effect, and found that it supported our hypotheses. On tasks where corrections were not relevant, our method had significantly lower regret ($p=0.001$); on tasks where corrections were relevant, there was no significant difference ($p=0.9991$). Figure \ref{fig:regret} plots the regret per task, and indeed our method was not inferior on tasks 1 and 3, and significantly better on tasks 2 and 4. We found analogous results on an ANOVA for the difference in learned weights from the optimal ones over time (see Figure \ref{fig:weight_path} for details). %%The factorial ANOVA analysis found a significant main effect for the method ($F(1,187)=76.43, p<0.0001$), and a significant interaction effect ($F(1,187)=33.3, p<0.0001$). A similar post-hoc analysis with Tukey HSD correction for multiple comparisons also supports our hypotheses. On tasks where corrections were not relevant, our method had significantly lower average weight paths over time ($p=0.0025$); on tasks where correction were relevant, however, there was no significant difference ($p=0.1584$). The same results are supported by Figure \ref{fig:delta_cost}, which plots the average length of $\hat{\theta}$ through weight space per task, and indeed our method was not significantly inferior for tasks 1 and 3, and significantly better on tasks 2 and 4. \annote{is there a less verbose way of talking about this second measure?}

\noindent\textbf{Subjective.}
We ran a repeated measures ANOVA on the results of our participant survey. We find that our method is not significantly different from the baseline in terms of task completion ($F(1,7)=0.88,p=0.348$) and task understanding ($F(1,7)=0.55, p=0.46$), which supports hypothesis H3. At the same time, participants significantly preferred our method in terms of reducing unintended learning ($F(1,7)=9.15,p=0.0046$), which supports out final hypothesis, H4.

{\renewcommand{\arraystretch}{1.5}% spaces out entries of table
\begin{table*}
 \centering
 \adjustbox{max width=\textwidth}{% makes table fit to page width
 \begin{tabular}{|c|l|c|c|c|}
 \hline
 & \multicolumn{1}{c|}{\textbf{Questions}} & \multicolumn{1}{c|}{\textbf{Cronbach's $\alpha$}} & \multicolumn{1}{c|}{\textbf{F-Ratio}} & \multicolumn{1}{c|}{\textbf{p-value}} \\
 \hline
 \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{task}}}} 
 & The robot accomplished the task in the way I wanted. & \multirow{2}{*}{0.94} & \multirow{2}{*}{0.88} & \multirow{2}{*}{0.348}\\
 & The robot was NOT able to complete the task correctly.  &&&\\
 \hline
 \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{undst.}}}} 
 & I felt the robot understood how I wanted the task done. & \multirow{2}{*}{0.95} & \multirow{2}{*}{0.55} & \multirow{2}{*}{0.46}\\
 &  I felt the robot did NOT know how I wanted the task done. &&&\\
 \hline
 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{unintend}}}} 
 & I had to undo corrections that I gave the robot. &&&\\
 & The robot wrongly updated its understanding about aspects of the task I did not want to change.  & \multirow{2}{*}{0.91} & \multirow{2}{*}{9.15} & \multirow{2}{*}{\textbf{0.0046}}\\
 & After I adjusted the robot, it continued to do the other parts of the task correctly.  &&&\\
 & After I adjusted the robot, it incorrectly updated parts of the task that were already correct. &&&\\
 \hline
 \end{tabular}
 }
 \strut % puts space between table and caption
 \label{table}
 \caption{Results of ANOVA on subjective metrics collected from a 7-point Likert-scale survey.} \label{tab:likert}
 \vspace{-5mm}
 \end{table*}}




==> old_demonstrations.tex <==
\section{Demonstrations}
\label{demonstrations}

\begin{itemize}
    \item Imagine a robot arm performing a household task, like moving a cup from the shelf onto your kitchen table. The robot wants to learn from a person's demonstrations how to best perform the task. For this purpose, the person gives one or a few demonstrations from which the robot infers the hidden reward function.
    \item Introduce notations for $x$, $\xi$, features, $\theta$.
    \item We commit to reward functions that are linear, using hand-engineered features.
    \item It is important to stress that the model misspecification issue we are trying to mitigate is quite general and does not exclusively affect objectives based on hand-crafted features: any model, by definition, will ultimately fail to capture the underlying motivation of some human actions. While it may certainly be possible, and desirable, to continually increase the complexity of the robot's model to capture a richer space of possible objectives, there will still be a need to account for the presence of yet-unlearned components of the true objective. In this sense, our work is \emph{complementary} to open-world objective modeling efforts.
    \item The cost function we are defining is parametrized by $\theta$, and penalizes effort while penalizing high feature values for large $\theta$:

\begin{equation}
    C_{\theta}(\xi) = \theta^T \phi(\xi) + \lambda \sum_{x^{\tau}\in\xi}\|x^{\tau}-x^{\tau-1}\|^2.
    \label{eq:cost}
\end{equation}

    \item Following \cite{von1945theory,baker2007goal,CORL}, we model the human as a noisily-rational agent that chooses actions which approximately minimize the robot's cost:

$$P(\xi_H|\theta,\beta) = \frac{e^{-\beta C_{\theta}(\xi_H)}}{\int_{\bar{\xi}_H}e^{-\beta C_{\theta}(\bar{\xi}_H)}d\bar{\xi}_H} = \frac{e^{-\beta (\theta^T \phi(\xi_H) + \lambda\|\xi_H\|^2)}}{\int_{\bar{\xi}_H}e^{-\beta (\theta^T \phi(\bar{\xi}_H) + \lambda\|\bar{\xi}_H\|^2)}d\bar{\xi}_H}$$

    \item Discuss that $\theta$ and $\beta$ overparametrize the problem. Hence we can think of $\theta$ as the direction of the intent and of $\beta$ as the norm, or magnitude, or rationality of the intent.
    \item Hence, we restrict our $\Theta$ space to the unit sphere.
    \item In this model, $\beta \in [0,\infty)$ is the rationality coefficient that determines the variance of the distribution over human actions. The coefficient $\beta$ adjusts how noisily the human picks $u_H$. When the person's correction is relevant, $\beta$ is large, while during irrelevant corrections $\beta$ is small, resulting in seemingly random behavior.
    \item Figure 3: For these last 3 points, perhaps we should brainstorm a figure that would give some geometric intuition of the $\theta$ and $\beta$ space.
    \item Clearly, this full computation of the observation model is intractable because of the integral in the denominator. How could we approximate this integral?
\end{itemize}

%The graphical model formulation in this case is a simple one: $\xi_H$ is the observed node, with two parents, $\theta$ and $\beta$, which are unobserved. Importantly, notice that when $\xi_H$ is observed, $\theta$ and $\beta$ could depend on each other, as our mathematical framework will reflect.

\subsubsection{Discretization}

\begin{itemize}
    \item we could discretize the trajectory space to approximate the integral as a summation (put in equation above but with summation instead of integral):
    $$\int_{\bar{\xi}_H}e^{-\beta (\theta^T \phi(\bar{\xi}_H) + \lambda\|\bar{\xi}_H\|^2)}d\bar{\xi}_H = \sum_{\bar{\xi}_H}e^{-\beta (\theta^T \phi(\bar{\xi}_H) + \lambda\|\bar{\xi}_H\|^2)}d\bar{\xi}_H$$
    \item explain how we choose the trajectory space: we pick $\theta$s of various magnitudes $\beta$ and get the optimum trajectories with respect to that $\beta\theta$ product. Overall we have about 2000 trajectories that span the space approximately uniformly.
    \item now we must do inference over $\theta$ and $\beta$:
    $$b(\theta; \beta) = \frac{P(\xi_H|\theta,\beta)P(\theta;\beta)}{\int_{\bar{\theta},\bar{\beta}}P(\xi_H|\bar{\theta},\bar{\beta})P(\bar{\theta};\bar{\beta})}$$
    \item we have another intractable integral, so we discretize the space of $\Theta$ and $\beta$ as well.
    \item we choose to do inference over $\beta\in \{0.01,0.03,0.1,0.3,1.0\}$ because a uniform over these values simulates an inverse exponential distribution over beta.
    \item explain how we choose the discrete space of $\theta$s to reason over. Uniform over a hypersphere?
    \item Figure 4: provide some intuition by looking at the heatmap of the posterior of $b(\theta; \beta)$. This figure has several parts to it:
    \begin{itemize}
        \item  We would have an example where the human's demonstration is correctly specified and very rational - expert behavior - (show image of demonstration + robot and human objective spaces), and we should see that the highest $\beta$ is active for the correct $\theta$. 
        \item  Next to it, We would have an example where the human's demonstration is correctly specified and noisy - noisy rational behavior - (show image of demonstration + robot and human objective spaces), and we should see that the highest $\beta$ is active for the correct $\theta$, but the heatmap isn't as strikingly focused as it was in the case of expert behavior. 
        \item Next to it we would have an example where the human's demonstration is misspecified (demonstration + R and H objective spaces), and we should see a larger spread out probability over the lower $\beta$ values for all the $\theta$s (heatmap below the demonstration image).
    \end{itemize}
    
    \item By having a belief $b(\theta; \beta)$, we can compute the expected $\beta$ value OR argmax OR have a P(misspecified|beta). To be determined how we can tell if we're misspecified or not.
    
    \item discuss downsides of this discrete method, which is that you can only get so much accuracy by discretizing everything, you need to reason over finitely many directions and magnitudes, which can be limiting. Since demonstration learning here is happening offline, we can afford to make the space of directions and magnitudes large anyway but it would be nice to have something that works directly on continuous values. And segue into this is why we do....:
\end{itemize}

\subsubsection{The Laplace Approximation}

\begin{itemize}
    \item IF WE USE CONTINUOUS TOO ONLY! MATH HERE IS TBD.
    \item provide intuition for mathematical terms: the idea that we care not only about the fact that human input is informative, but also about how informative it is.
    \item One option is to employ the Laplace approximation, which essentially approximates the integral by its mode. Let's walk through the set-by-step derivation. (I have attached this here below in comments; we might want to have it as an appendix in the paper though.)
    \item By replacing this new approximate integral, our observation model becomes:

\begin{equation}
    P(\xi_H|\theta,\beta) = e^{-\beta (\theta^T (\phi(\xi_H)-\phi(\xi_H^*)) + \lambda(\|\xi_H\|^2-\|\xi_H^*\|^2))} \sqrt{\frac{\beta^k |H_{\xi_H^*}|}{(2\pi)^k}}.
    \label{eq:laplace_obs}
\end{equation}

    \item Now, using this observation model, we can retrieve the posterior belief by using and MAP/MLE... (tbd)
\end{itemize}


%For our cost $C_{\theta}(\xi_H)$ as defined in Equation \ref{eq:cost}, we perform a second-order Taylor series expansion around the optimal $\xi_H^*$:

%$$C_{\theta}(\xi_H) \approx C_{\theta}(\xi_H^*) + \nabla C_{\theta}(\xi_H^*)^T(\xi_H - \xi_H^*) + \frac{1}{2}(\xi_H - \xi_H^*)^T\nabla^2C(\xi_H^*)(\xi_H - \xi_H^*)$$

%Since our cost function has a global minimum, at the optimum we have that $\nabla C_{\theta}(\xi_H^*) = 0$, and our integral becomes:

%$$\int_{\bar{\xi}_H}e^{-\beta C_{\theta}(\bar{\xi}_H)}d\bar{\xi}_H \approx e^{-\beta C_{\theta}(\xi_H^*)} \int_{\bar{\xi}_H}{e^{- \frac{\beta}{2}(\bar{\xi}_H - \xi_H^*)^TH_{\xi_H^*}(\bar{\xi}_H - \xi_H^*)}d\bar{\xi}_H}, $$

%where $H_{\xi_H^*}$ is the Hessian of the cost function around $\xi_H^*$. Notice that the second integral can be evaluated as a Gaussian integral:

%$$\int_{\bar{\xi}_H}{e^{- \frac{\beta}{2}(\bar{\xi}_H - \xi_H^*)^TH_{\xi_H^*}(\bar{\xi}_H - \xi_H^*)}d\bar{\xi}_H} = \sqrt{\frac{(2\pi)^k}{\beta^k |H_{\xi_H^*}|}},$$

%where $k$ is the number of features in the robot's hypothesis space. As such, our integral in the denominator is finally approximated as:

%$$\int_{\bar{\xi}_H}e^{-\beta C_{\theta}(\bar{\xi}_H)}d\bar{\xi}_H \approx e^{-\beta C_{\theta}(\xi_H^*)} \sqrt{\frac{(2\pi)^k}{\beta^k |H_{\xi_H^*}|}}. $$


==> pHRI.tex <==
\section{Physical Corrections}
\label{phri}

\abnote{This is the math from the CoRL paper, pasted in bullets. In the journal version, the language will change a bit to make references to the discrete case, but the general flow of ideas should be similar to CoRL.}

\begin{itemize}
    \item We consider settings where a robot is collaborating with a person to perform everyday tasks by learning from pHRI, but their feature spaces might not be shared. When the robot receives human input, it should be able to reason about the relevance of the action and replan its trajectory accordingly.
    \item \noindent\textbf{A Graphical Model for Correction Relevance.} Let $x$ describe the robot's state (joint position and velocity) and $u_R$ the robot's action (the control torque it applies). By default, the robot generates actions via an impedance controller to track a trajectory $\xi_R = x^{0:T} \in \Xi$. This trajectory is optimal with respect to the robot's objective which is encoded as a linear combination of features of the state, $\phi(x^t)$ \cite{abbeel2004apprenticeship,maxent}. The robot might adapt its objective over time, which means it replans and tracks a new trajectory corresponding to its understanding of the objective at the current time $t$ by solving $\xi_R^t = \arg\min_{\xi} {\hat\theta}^\top\Phi(\xi)$. Here  $\Phi(\xi) = \sum_{x^{\tau}\in\xi} \phi(x^{\tau})$ is the total feature count along a particular trajectory $\xi$, and $\hat\theta \in \Theta$ represents the current weights on these features. 
    \item At any timestep during the trajectory execution, the human may physically interact with the robot, inducing a joint torque, $u_H$. Following \cite{von1945theory,baker2007goal,CORL}, we model the human as a noisily-rational agent that chooses actions which approximately minimize the robot's cost:

\begin{equation}
P(u_H \mid \xi_R; \beta, \theta) = \frac{e^{-\beta ({\theta}^\top\Phi(\xi_H) + \lambda\|u_H\|^2)}}{\int e^{-\beta ({\theta}^\top\Phi(\bar{\xi}_H) + \lambda\|\bar{u}_H\|^2)}d\bar{u}_H}\enspace.
\label{eq:boltzmann}
\end{equation}

\item  Lastly, in this work, we compute $\xi_H$ by deforming the robot's current trajectory $\xi_R$ in the direction of $u_H$ via $\xi_H = \xi_R + \mu A^{-1}U_H$ \cite{CORL}. Here, $\mu>0$ scales the magnitude of the deformation, $A$ defines a norm on the Hilbert space of trajectories and dictates the deformation shape \cite{deformation}, and $U_H=u_H$ at the current time and $U_H=0$ otherwise\footnote{We used a norm $A$ based on acceleration, consistent with \cite{CORL}, but other norm choices are possible as well.}. When choosing actions, the human is modeled as trading off between inducing a good trajectory $\xi_H$ with respect to~$\theta$, and minimizing their effort. 

\item Ideally, with this model of human actions we would perform inference over both the rationality coefficient $\beta$ and the parameters $\theta$ by maintaining a joint Bayesian belief $b(\beta, \theta)$, similarly to what we did in the demonstrations case. Our probability distribution over $\theta$ would automatically adjust for relevant corrections, whereas for irrelevant ones the robot would stay closer to its prior on $\theta$: the robot would implicitly realize that there is a better $u_H$ for each possible $\theta$, and therefore no $\theta$ explains the correction. 

\item Figure 5: Could have the same figure at Figure 4, but I don't have code that currently does this discrete beta for pHRI. Or, I have code, but I haven't tested it on pHRI in a year. If we think this figure could be valuable and worth the time, I can look into making that work.

\item Unfortunately, this is not possible in real time given the continuous and possibly high-dimensional nature of the weight-space, $\Theta$.

\item The fact that we are aiming for real-time is the reason why we can't do the same math we were doing above, in the demonstrations case, which is why here we need an approximation.

\item To alleviate the computational challenge of performing joint inference over $\beta$ and $\theta$, we introduce a binary variable $r \in \{0,1\}$ which (a) indicates interaction relevance, and (b) allows us to split inference over $\beta$ and $\theta$ into two separate computations. When $r=1$, the interaction appears less noisy (i.e. $\beta$ is large) and the human's desired modification of the robot's behavior can be well explained by \emph{some} feature weight vector $\theta \in \Theta$. As a result, the interaction $u_H$ is likely to be efficient for the cost encoded by this $\theta$. Conversely, when $r=0$, the interaction appears noisy (i.e. $\beta$ is small) and the person is correcting some feature(s) that the robot does not have access to. Thus, the interaction $u_H$ is substantially less likely to be efficient for any cost expressible within the space $\Theta$.

\begin{figure*}
\centering
\includegraphics[width=0.85\textwidth]{figures/graphical_model.pdf}
\caption{(a) In the complete graphical model, $u_H$ is an observation of the true objective ($\theta$) and rationality coefficient ($\beta$);
inference over $\theta$ is intractable.(b) We use the proxy variable $\Phi(\xi_H)$ to first estimate $\beta$. (c) We interpret the estimate $\hat{\beta}$ as an indirect observation of the unobserved $r$, which we then use for the $\theta$ estimate.}
\label{fig:graphical_models}
\end{figure*}

\item Figure 6: Overall, this forms the graphical model in \ref{fig:graphical_models}a, with $P(u_H \mid \xi_R; \beta, \theta)$ defined above, and the distribution $P(\beta \mid r)$ (describing what $\beta$ we expect under relevant or irrelevant corrections) to be learned empirically. Next, we simplify the problem to enable real time computation while preserving the benefit of automatically adjusting the learning depending on relevance. 

\item \noindent\textbf{Approximate Inference.} We simplify inference by leveraging a proxy variable $\Phi(\xi_H)$---the feature values of the corrected trajectory $\xi_H$---to split the problem into two stages. Rather than looking at how relevant $u_H$ is overall, we estimate rationality $\beta$ (and therefore relevance $r$) based on how efficiently $u_H$ produced the feature values of $\Phi(\xi_H)$. If there is a more efficient correction that would induce $\Phi(\xi_H)$, this suggests that the correction was not relevant to the robot's hypothesis space. Then, armed with an estimate of relevance, we infer $\theta$ from $\Phi(\xi_H)$. 
\item These two steps are captured by the two simplified graphical models in Figure \ref{fig:graphical_models}b and Figure \ref{fig:graphical_models}c. The first relates $u_H$ to $\beta$, $\xi_R$, and the induced feature values $\Phi(\xi_H)$ by modeling that $u_H$ should achieve the $\Phi(\xi_H)$ with minimal effort. The conditional probability in this Bayes net is: 

\vspace{-0.5cm}
\begin{equation}
	P(u_H \mid \beta, \Phi(\xi_H), \xi_R) = \frac{e^{-\beta( \|u_H\|^2)}}{\int e^{-\beta( \|\bar{u}_H\|^2+ \lambda\|\Phi(\bar{\xi}_H) - \Phi(\xi_H)\|^2 )}d\bar{u}_H}\enspace,\label{eq:bayesnetb_model}
\end{equation}

\item where the cost function is $\beta( \|u_H\|^2 + \lambda\|\Phi(\xi_H) - \Phi(\xi_H)\|^2)$, with $\lambda\|\Phi(\bar{\xi}_H) - \Phi(\xi_H)\|^2 $ a strong penalty on deviating from the induced features (this penalty is 0 in the numerator since the observed $\Phi(\xi_H)$ is exactly the one induced by $u_H$). This will enable us to estimate a $\hat{\beta}$ from the observed $u_H$.

\item The second simplified graphical model (Figure \ref{fig:graphical_models}c) relates the induced feature values $\Phi(\xi_H)$ to $\theta$ as a function of the relevance. When $r=1$, the induced features should have low cost with respect to $\theta$; when $r=0$, the induced features \emph{do not depend on $\theta$}, and we model them as Gaussian noise centered at the current robot trajectory feature values:
\begin{equation}
P(\Phi(\xi_H) \mid \theta, r) = \begin{cases} \frac{e^{-\theta^\top\Phi(\xi_H)}}{\int e^{-\theta^{\top}\Phi(\tilde{\xi}_H)} d\tilde{\xi}_H} ,& r=1 \\ \left(\frac{\lambda}{\pi}\right)^\frac{k}{2} e^{-\lambda ||\Phi(\xi_H)-\Phi(\xi_R)||^2} ,& r=0 \end{cases}
\label{eq:bayesnetc_model}
\end{equation}
with the constant in the $r=0$ case corresponding to the normalization term of the normal distribution.

\item Finally, this graphical model also relates the estimated $\hat{\beta}$ from the first simplified model to $r$ by a $P(\hat{\beta} \mid r)$. We fit this distribution from controlled user interaction samples where we know $r$. For each sample interaction, we compute a $\hat{\beta}$ (using Equation \ref{eq:beta_map} below) and label it with the corresponding binary $r$ value. 

\item Figure 7: We fit a chi-squared distribution to these samples to obtain the probability distributions for $P(\hat{\beta} \mid r=0)$ and $P(\hat{\beta} \mid r=1)$. The resulting distribution fits are shown in Figure \ref{fig:histograms}.

\item \noindent\textbf{Estimating $\beta$.} The integral in Equation \ref{eq:bayesnetb_model} is computationally prohibitive, but we can approximate it via a Laplace approximation (detailed in Appendix \ref{app:laplace}): 

\begin{equation}
	P(u_H \mid \beta, \Phi(\xi_H), \xi_R) \approx \frac{e^{-\beta(  \|u_H\|^2)}}{ e^{-\beta( \|{u_H^*}\|^2 + \lambda\|\Phi({\xi_H^*}) - \Phi(\xi_H)\|^2)}}\sqrt{\frac{\beta^k|H_{u^*_H}|}{2\pi^k}}
\enspace,
\label{eq:laplace}
\end{equation}
where $k$ is the action space dimensionality and $H_{u_H^*}$ is the Hessian of the cost function around $u_H^*$. We obtain the optimal action $u_H^*$ by solving the constrained optimization problem:
%
\begin{equation}
\begin{aligned}
& \underset{u}{\text{minimize}}
& & \|u\|^2 \\
& \text{subject to}
& & \Phi(\xi_R+\mu A^{-1}U) - \Phi(\xi_H) = 0.
\end{aligned}
\label{opt:optimal_uH}
\end{equation}

\item Notice that by formulating the problem as a constrained optimization, the $\lambda$-term in Equation \ref{eq:laplace} is close to 0 and vanishes, so the final conditional probability becomes:

\begin{equation}
	P(u_H \mid \beta, \Phi(\xi_H), \xi_R) = e^{-\beta(\|u_H\|^2-\|u_H^*\|^2 )}\sqrt{\frac{\beta^k|H_{u^*_H}|}{2\pi^k}}\enspace.
\label{eq:laplace2}
\end{equation}

\item We can obtain an estimate of the rationality coefficient via a maximum likelihood estimate:

\begin{gather}
	\hat{\beta} = \arg\max_{\beta} \{\log(P(u_H \mid \beta, \Phi(\xi_H), \xi_R))\} =\\ = \arg\max_{\beta} \{-\beta(\|u_H\|^2-\|u_H^*\|^2 ) + \log(\sqrt{\frac{\beta^k|H_{u^*_H}|}{2\pi^k}})\}
\end{gather}

and setting the gradient to zero:

\begin{equation}
	\hat{\beta} = \frac{k}{2(\|u_H\|^2-\|u_H^*\|^2)}\enspace.
\label{eq:beta_map}
\end{equation}

\item \noindent\textbf{Intuitive Interpretation of $\hat{\beta}$.} The estimator above yields a high value when the difference between $u_H$ and $u_H^*$ is small, i.e. the person's correction achieves the induced features $\Phi(\xi_H)$ efficiently. For instance, if $\xi_H$ brings the robot closer to the table, and $u_H$ pushes the robot straight towards the table, $u_H$ is an efficient way to induce those new feature values. However, when there is a much more efficient alternative (e.g. when the person pushes mostly sideways rather than straight towards the table), $\hat{\beta}$ will be small. Efficient ways to induce the feature values will suggest relevance, inefficient ones will suggest irrelevance (i.e. there is something else that explains the correction).

\item \noindent\textbf{Estimating ${\theta}$.}
Lastly, we can infer a new $\theta$ estimate based on the model from Figure  \ref{fig:graphical_models}c.
We do this tractably by interpreting the estimate $\hat\beta$ obtained from \eqref{eq:beta_map} as an indirect observation of the unknown variable $r$.
We empirically characterize the conditional distribution $P(\hat\beta\mid r)$, and then combine the learned likelihood model with an initial uniform prior $P(r)$ to maintain a Bayesian posterior on $r$ based on the evidence $\hat\beta$ constructed from human observations at deployment time, $P(r \mid \hat\beta) \propto P(\hat\beta \mid r) P(r)$.

\item Further, since we wish to obtain a posterior estimate of the human's objective $\theta$, we use the model from Figure  \ref{fig:graphical_models}c to obtain the posterior probability measure
\begin{equation}\label{eq:theta_from_beta_hat}
P(\theta \mid \Phi(\xi_H),\hat\beta) \propto \sum_{r \in \{0,1\} } P\big(\Phi(\xi_H) \mid \theta, r\big) P(r \mid \hat\beta) P(\theta)
\enspace.
\end{equation}

\item Following \cite{CORL}, we approximate the partition function in the human's policy  \eqref{eq:bayesnetc_model} by the exponentiated cost of the robot's original trajectory, thereby obtaining
\begin{equation}
P(\Phi(\xi_H) \mid \theta, r=1) = 
	e^{-\theta^\top\big(\Phi(\xi_H)-\Phi(\xi_R)\big)}\enspace. 
\label{eq:bayesnetc_with_constants}
\end{equation}

\item We also consider a Gaussian prior distribution of $\theta$ around the robot's current estimate $\hat\theta$:
\begin{equation}
P(\theta) = \frac{1}{(2\pi\alpha)^\frac{k}{2}} e^{-\frac{1}{2\alpha} ||\theta-\hat{\theta}||^2}
\enspace.
\end{equation}

\item The maximum-a-posteriori estimate of the human's objective $\theta$ is therefore the solution maximizer of

\begin{gather}\begin{aligned}\label{eq:posterior_theta}
P(\theta) \Big[ P(r=1 \mid \hat\beta)P\big(\Phi(\xi_H)\mid\theta,r=1\big) + \\ + P(r=0 \mid \hat\beta)P\big(\Phi(\xi_H)\mid \theta,r=0\big) \Big] \\
     = \frac{1}{(2\pi\alpha)^\frac{k}{2}}
e^{-\frac{1}{2\alpha}||\theta-\hat{\theta}||^2}
   \Big[ P(r=1 \mid \hat\beta) e^{-\theta^\top\big(\Phi(\xi_H)-\Phi(\xi_R)\big)}\\ + P(r=0 \mid \hat\beta) \left(\frac{\lambda}{\pi}\right)^\frac{k}{2} e^{-\lambda||\Phi(\xi_H)-\Phi(\xi_R)||^2}\Big]
\enspace.
\end{aligned}\end{gather}

\item Differentiating \eqref{eq:posterior_theta} with respect to $\theta$ and equating to 0 gives the maximum-a-posteriori update rule:
\begin{gather}\label{eq:theta_update}
\hat\theta' = \hat\theta - \alpha \frac{P(r=1 \mid \hat\beta) e^{-\hat\theta'^\top\big(\Phi(\xi_H)-\Phi(\xi_R)\big)}}
{P(r=1 \mid \hat\beta) e^{-\hat\theta'^\top\big(\Phi(\xi_H)-\Phi(\xi_R)\big)} +
P(r=0 \mid \hat\beta) \left(\frac{\lambda}{\pi}\right)^\frac{k}{2} e^{-\lambda||\Phi(\xi_H)-\Phi(\xi_R)||^2}}
\big(\Phi(\xi_H)-\Phi(\xi_R)\big)
\enspace.
\end{gather}

\item We note that due to the coupling in $\hat\theta'$, the solution to \eqref{eq:theta_update} is non-analytic and can instead be obtained via classical numerical approaches like Newton-Raphson or quasi-Newton methods.

\item In previous objective-learning approaches including \cite{CORL} and \cite{maxent}, it is implicitly assumed that all human actions are fully explainable by the robot's representation of the objective function space ($r=1$), leading to the simplified update
\begin{equation}\label{eq:corl_update}
\hat\theta' = \hat\theta - \alpha
\big(\Phi(\xi_H)-\Phi(\xi_R)\big)
\enspace,
\end{equation}
which can be easily seen to be a special case of \eqref{eq:theta_update} when $P(r=0 \mid \hat\beta)\equiv 0$.
Our proposed update rule therefore \emph{generalizes} commonly-used objective-learning formulations to cases where the human's underlying objective function is not fully captured by the robot's model.
We expect that this extended formulation will enable learning that is more robust to misspecified or incomplete human objective parameterizations. Once we obtain the $\hat{\theta}'$ update, we replan the robot trajectory in its 7-DOF configuration space with an off-the-shelf trajectory optimizer\footnote{We provide an open-source implementation of our method \href{https://github.com/andreea7b/beta_adaptive_pHRI}{here}. We used TrajOpt \cite{trajopt}, which is based on sequential quadratic programming and uses convex-convex collision checking.}. 

\item \noindent\textbf{Intuitive Interpretation of $\hat{\theta}$.} The update rule changes the weights in the objective in the direction of the feature difference as well, but how much it does so depends on the probability assigned to the correction being relevant. At one extreme, if we know with full certainty that the correction is relevant, then we do the full update as in traditional objective learning. But crucially, at the other extreme, if we know that the correction is irrelevant, we do not update at all and keep our prior belief.

\end{itemize}

